Spin-polarization of the neutron ocean in magnetar crusts

Magnetars, neutron stars harboring the strongest magnetic fields known in the Universe, are associated with a broad range of observational phenomena, from giant flares to fast radio bursts, and have also been proposed as potential sites of heavy-element nucleosynthesis. These phenomena are thought to be closely linked to the structure and composition of magnetar crusts. The outer crust consists of fully ionized nuclei embedded in a degenerate electron gas, while the inner crust additionally contains free neutrons. We investigate how strong magnetic fields modify magnetar crusts, accounting for the spin polarization of free neutrons. Arising from the coupling between the magnetic field and the neutron magnetic moment, neutron spin polarization lowers both the pressure and matter density marking the boundary between the outer and inner crusts for magnetic field strengths $B \gtrsim 10^{17}~\mathrm{G}$. As a consequence, the outer crust becomes thinner, the formation of the superheavy nuclei predicted in previous studies is suppressed, and the neutron ocean permeating the inner crust becomes spin-polarized. These effects may have important implications for the diverse manifestations of magnetars and for $r$-process nucleosynthesis in the ejecta of magnetar giant flares.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
